CLIP-FLow: Contrastive Learning by semi-supervised Iterative Pseudo labeling for Optical Flow Estimation

Synthetic datasets are often used to pretrain end-to-end optical flow networks, due to the lack of a large amount of labeled, real-scene data. But major drops in accuracy occur when moving from synthetic to real scenes. How do we better transfer the knowledge learned from synthetic to real domains? To this end, we propose CLIP-FLow, a semi-supervised iterative pseudo-labeling framework to transfer the pretraining knowledge to the target real domain. We leverage large-scale, unlabeled real data to facilitate transfer learning with the supervision of iteratively updated pseudo-ground truth labels, bridging the domain gap between the synthetic and the real. In addition, we propose a contrastive flow loss on reference features and the warped features by pseudo ground truth flows, to further boost the accurate matching and dampen the mismatching due to motion, occlusion, or noisy pseudo labels. We adopt RAFT as the backbone and obtain an F1-all error of 4.11%, i.e. a 19% error reduction from RAFT (5.10%) and ranking 2$^{nd}$ place at submission on the KITTI 2015 benchmark. Our framework can also be extended to other models, e.g. CRAFT, reducing the F1-all error from 4.79% to 4.66% on KITTI 2015 benchmark.

==> 0-abs.tex <==
%%%%%%%%%%%%%%%%%%%
%% Abstract %%%%%%%
%%%%%%%%%%%%%%%%%%%

%Recent semi-supervised learning (SSL) works have shown to be very effective in learning inherent visual features for a range of computer vision tasks. Its application particularly becomes indispensable in dense prediction tasks where having accurate and optimum amount of ground-truth is cumbersome, for a fully supervised training. Contemporary works have employed SSL for Vision Transformers(VITs) and ResNet based architecture to achieve state-of-arts results. In this work, we focus on finding the optimum training strategy, along with employing SSL approaches such as contrastive learning and pseudo labelling, to optical flow estimation. In particular, we train our model on the huge unlabeled KITTI Raw dataset, thus bridge the gap between the real captured scene data and synthetic data. For this we leverage the well known RAFT model as a base architecture to prove generalizability of our method. Despite its simplicity and with no obvious increase in the size of the trainable model, we significantly improve the performance for the flow estimation task. Finally, we evaluate our proposed method on KITTI test, beating all existing \textit{F1-all error} numbers with a score of 4.11.

%Recent semi-supervised learning (SSL) works have shown to be very effective in learning inherent visual features for a range of computer vision tasks. Its application particularly becomes indispensable in dense prediction tasks where having accurate and a large amount of ground-truth is cumbersome, for a fully supervised training. Contemporary works have employed SSL for Vision Transformers(VITs) and ResNet based architecture to achieve state-of-arts results. In this work, we focus on finding the optimum training strategy, along with employing SSL approaches such as contrastive learning and pseudo labelling, to optical flow estimation. In particular, we train our model on the huge unlabeled KITTI Raw dataset, thus bridge the gap between the real captured scene data and synthetic data. For this we leverage the well known RAFT model as a base architecture to prove generalizability of our method. Despite its simplicity and with no obvious increase in the size of the trainable model, we significantly improve the performance for the flow estimation task. Finally, we evaluate our proposed method on KITTI test, beating all existing \textit{F1-all error} numbers with a score of 4.11.


%\ccjscomments{Will rewrite???}
Semi-supervised learning has been presenting promising results in many 2D computer vision tasks, \eg, image classification and segmentation. But for optical flow, a dense prediction task with strong geometry priors, less studies have been proposed due to the difficulty of self-supervised training without dense supervision from ground truth labels. To this end, we propose \ourname{}, a semi-supervised framework for optical flow, which boosts image representation learning with an explicit contrastive flow loss for accurate matching, together with an iterative pseudo labeling strategy to leverage the ubiquitous, unlabeled data by generating pseudo ground truth labels to facilitate dense optical flow training. In particular, we train our model on a large amount of unlabeled KITTI Raw data, instead of the synthetic data, bridging the domain gap between the real world scenes and synthetic ones. We adopt RAFT as a backbone architecture and obtain non-trivial improvement. Despite its simplicity and with no obvious increase in the size of the trainable model, we significantly improve the performance for the flow estimation task. We evaluate our proposed method on KITTI test, beating all existing \textit{F1-all error} numbers with a score of 4.11. Further more, we demonstrate the proposed training strategy can be extended to other models like CRAFT, and further improve the F1-all error score on KITTI test for a big margin.  


==> algo_1_v0.tex <==
\iffalse
\begin{algorithm}
%\caption{ Semi-supervised Iterative Flow Refinement }
\caption{Semi-supervised iterative pseudo labeling for optical flow estimation}
\label{alg:SSL_Train}
\begin{algorithmic}[1]
\Require $R_i$ \Comment{Pretrained initial RAFT Model}
\Require $K_R, K_F$ \Comment{KITTI raw and flow dataset}
\Require $R_f$ \Comment{RAFT model with contrastive loss}
\While{True}
\State $steps \gets 0$
\State $Pseudo_{GT} = R_i(K_R)$
\State $R_t \gets R_f$
\While{$steps \leq threshold$}
\State $loss = loss\_function(R_t(K_R), Pseudo_{GT})$
\State $R_t = update(R_t)$
\EndWhile
\State $steps \gets 0$
\State $n = cross\_val(R_t, K_F)$ \Comment {Get training steps}
\While{$steps \leq n$}
\State $R_t = finetune(R_t, K_F)$
\EndWhile
\State $R_i = R_t$ \Comment {Update $R_i$}
\EndWhile
\end{algorithmic}
\end{algorithm}
\fi


==> tmp-tables.tex <==
\iffalse
\begin{table}[!h]
\begin{subtable}{0.5\linewidth}
\begin{tabular}{ c |c | c | c }
\centering
\hline
\footnotesize{iteration} & \footnotesize{steps} & \footnotesize{F1-all(val)} & \footnotesize{F1-all(test)} \\
\hline
\footnotesize{1st} &\footnotesize{1.2m}&\footnotesize{  3.99 } &\footnotesize{4.38} \\
\footnotesize{2nd} &\footnotesize{1.2m}&\footnotesize{  3.42 } &\footnotesize{-*} \\
\footnotesize{3rd} &\footnotesize{1.2m}&\footnotesize{  3.18 } &\footnotesize{4.13} \\
\footnotesize{3rd} &\footnotesize{5m}&\footnotesize{  2.78 } &\footnotesize{4.11} \\
 \hline
\end{tabular}
\caption{The comparison of  F1-all error on KITTI-Flow-Val and KITTI-Flow-test at different iteration and different training steps. \tiny{*Each group just have 3 chances to upload their testing results on KITTI-Flow-test lead-board. Although we didn't have all the F1-all error score from KITTI-Flow-test lead-board, we can clear see the trend: the KITTI-Flow-test F1 error score is highly consistent with the one of KITTI-Flow-Val.}} 
\label{table:iterationresults}
\end{subtable}\hfill

\begin{subtable}{0.5\linewidth}
\begin{tabular}{l | c |c }
\centering
\hline
 %\diagbox{Models (at step 1.2m) } 
 {Models (at step 1.2m) } 
 & \footnotesize{F1-all(validation)} &\footnotesize{F1-all(test)} \\ 
 \hline 
 \footnotesize{ RAFT+IP }  &\footnotesize{4.531}  & \footnotesize{4.48}  \\  
 \footnotesize{RAFT+IP+Coord}  & \footnotesize{4.45}  & \footnotesize{-*}  \\
 \footnotesize{RAFT+IP +CC}  & \footnotesize{3.99}  & \footnotesize{4.38}    \\
\hline
\end{tabular}
\caption{ The comparison of F1-all error KITTI-Flow-Val and
KITTI-Flow-test for different model, RAFT+IP is the original raft model structure train on KITTI-Raw use our proposed iterative pseudo labeling strategy, related with the light blue curve in Fig. \ref{image:ablation}, RAFT+IP+Coord is original raft model only add the coordinate embedding train on KITTI-Raw use our proposed iterative pseudo labeling strategy, related with the dark blue curve in Fig. \ref{image:ablation}, and RAFT+IP+C+C is the complete proposed method RAFT-CF model train on KITTI-Raw use our proposed iterative pseudo labeling strategy, related with pink curve in Fig. \ref{image:ablation}.  *To be noted that we can't submit all the ablation results to KITTI-Flow-test leadboard because every research group only has 3 chance per month. We can still tell the trend from the F1 error score in KITTI-Flow-Val given that the F1 error score is very consistence in KITTI-Flow-test and KITTI-Flow-Val  in our experiments.} 

\centering
\end{subtable}
\end{table}
\label{table:ablation}
\if
